Demystification and Near-perfect Estimation of Minimum Gas Limit and Gas Used for Ethereum Smart Contracts

The Ethereum blockchain has a \emph{gas system} that associates operations with a cost in gas units. Two central concepts of this system are the \emph{gas limit} assigned by the issuer of a transaction and the \emph{gas used} by a transaction. The former is a budget that must not be exhausted before the completion of the transaction execution; otherwise, the execution fails. Therefore, it seems rather essential to determine the \emph{minimum gas limit} that ensures the execution of a transaction will not abort due to the lack of gas. Despite its practical relevance, this concept has not been properly addressed. In the literature, gas used and minimum gas limit are conflated. This paper proposes a precise notion of minimum gas limit and how it can differ from gas used by a transaction; this is also demonstrated with a quantitative study on real transactions of the Ethereum blockchain. Another significant contribution is the proposition of a fairly precise estimator for each of the two metrics. Again, the confusion between these concepts has led to the creation of estimators only for the gas used by a transaction. We demonstrate that the minimum gas limit for the state of the Ethereum blockchain (after the block) $t$ can serve as a near-perfect estimation for the execution of the transaction at block $t + \Delta$, where $\Delta \leq 11$; the same holds for estimating gas used. These precise estimators can be very valuable in helping the users predict the gas budget of transactions and developers in optimising their smart contracts; over and underestimating gas used and minimum gas limit can lead to a number of practical issues. Overall, this paper serves as an important reference for blockchain developers and users as to how the gas system really works.

==> old_conclusion.tex <==
The main contribution of this paper is a more precise account of how the Ethereum gas system works. Although both the \textit{eth\_estimateGas()} and \textit{debug\_traceCall()} functions are present in most estimators currently available, the official documentation for both does not describe in detail how they actually behave. We have analysed and detailed the behaviour of these functions; also, through our experiments, we report that, despite the overall high precision of both functions, each one tends to lose accuracy as the time/block intervals ($\Delta$) between their estimates and the insertion of transactions into the blockchain increase. In addition, we identified a list of opcodes that are dependent on the block state and reported results indicating that the precision of the \textit{eth\_estimateGas()} and \textit{debug\_traceCall()} functions is also consistently affected by the presence of these opcodes.

In answering \gls{rq1} and \gls{rq2}, we suggest specific scenarios in which the \textit{eth\_estimateGas()} and \textit{debug\_traceCall()} functions are expected to perform similarly to a perfect estimator. Specifically, we find that both functions begin to suffer significant precision degradation when the interval between their estimates and the insertion of transactions into the blockchain exceeds 10 blocks (approximately 2 minutes) for transactions that do not contain block state-dependent opcodes and at any block interval for transactions that do contain such opcodes. This way, we clarify how to use these functions to estimate the \glspl{mgl} and \glspl{gu} by transactions, respectively, opening the door for users and developers to use them more efficiently, taking their peculiarities into account.

Another important hypothesis was that \gls{mgl} and \gls{gu} are two distinct concepts, although they are often confused and conflated in the current literature. More specifically, we define that, while \gls{gu} refers to the number of gas units that a given transaction consumes when being executed, \gls{mgl} determines the number of gas units that the transaction requires to be executed. Both via some subtle examples (in Section~\ref{section:minimum-gas-limit-vs-gas-used}) and the Experiment E3 (Section~\ref{section:minimum-gas-limit-vs-gas-used-experiment}), we demonstrate that there are situations where the \gls{mgl} differs from the \gls{gu} of transactions. 

Particularly, analysing the \glspl{mgl} and the \glspl{gu} by transactions, we identified significant differences between the distributions of the two metrics. To address \gls{rq3}, we present results that indicate that these distributions have significantly different shapes, regardless of whether the transactions contain block state-dependent opcodes. Furthermore, our experiments suggest a linear relationship between \glspl{mgl} and \glspl{gu} in transactions that do not contain block state-dependent opcodes. By confirming that \glspl{mgl} and \glspl{gu} are two distinct concepts, this work paves the way for researchers and developers to propose new solutions that, considering this distinction, are more accurate in estimating both the \gls{mgl} and the \gls{gu} by transactions.



%\subsection{Contributions} %\label{subsection:contributions}
%
%By presenting the \glspl{mgl} and \glspl{gu} as two distinct concepts, demonstrating with examples how their values can diverge, and reporting results that reveal significant differences between their value distributions, this work paves the way for researchers and developers to propose new solutions that, considering this distinction, are more accurate in estimating both the minimum gas limit and the gas used by transactions.

%Although both the \textit{eth\_estimateGas()} and \textit{debug\_traceCall()} functions are present in most estimators currently available, the official documentation for both does not describe in detail how they work. By clarifying the functionality of these functions, this work opens the door for users and developers to use them more efficiently, taking their peculiarities into account.

%The experiments in this work demonstrated how the precision of gas estimators can be affected both by the presence of block state-dependent opcodes in transactions and by different time/block intervals between their estimates and the insertion of transactions into the blockchain. In addition to presenting scenarios in which the \textit{eth\_estimateGas()} and \textit{debug\_traceCall()} functions can be used with a higher level of confidence, this understanding provides a foundation for new research aimed at understanding how the accuracy of gas estimators can be influenced by the presence of specific opcodes in transactions and by the delay in including these transactions in the blockchain.


%\subsection{Limitations} %\label{subsection:limitations}

We also emphasise some limitations of our work. As part of our experimental project, we presented a list of block state-dependent opcodes; throughout the experiments, we reported results suggesting the influence of such opcodes on the accuracy of gas estimators. Although we identified this relationship between block state-dependent opcodes and the precision of gas estimators, we did not conduct a detailed study on how each of these opcodes can individually influence gas estimates.

Furthermore, we selected transactions belonging to a single fork that were allocated at the zero index position in their respective blocks. This measure ensured that all selected transactions were included in the blockchain according to the same consensus rules and allowed us to associate the state of the \gls{evm} in a block of height $b - 1$ with a transaction selected from a block $b$. Considering that the Ethereum blockchain currently accumulates more than 2 million blocks, each with multiple transactions, one should be aware that the scope of the experiments conducted in this work, although containing tens of thousands of transactions, represents a relatively small percentage of the total transactions stored on the Ethereum blockchain. Furthermore, the dynamic nature of Ethereum updates can introduce consistent changes to its gas system, requiring further investigation to verify if the conclusions of this work will still be applicable.

%\subsection{Future Work} %\label{subsection:future-work}

The results and limitations presented in this work can drive various future research directions. We present some of them below:

\begin{itemize}

    \item Detailed analysis of the behaviour of block state-dependent opcodes, with the aim of understanding how each of these opcodes can individually impact the precision of gas estimators.

    \item Expansion of the experimental scope, including transactions from other forks, with varied indices and positions within blocks, while also considering different levels of delay in the inclusion of these transactions on the blockchain.

    \item Development of adaptive mechanisms, based on machine learning or other approaches, aiming to both improve the precision of gas estimators in transactions containing block state-dependent opcodes and maintain this precision even in the presence of delays in the inclusion of these transactions on the blockchain.

    \item In-depth investigation into the relationship between the \gls{mgl} and \gls{gu} by transactions, especially in cases where these transactions do not contain block state-dependent opcodes, with the goal of proposing dual-approach gas estimators capable of deriving the \gls{mgl} estimate from the \gls{gu} by transactions and vice versa.
    
\end{itemize}

==> old_intro.tex <==
Ethereum is an open-source, decentralized, distributed computing platform \cite{Buterin:2014}, designed based on the blockchain technology originally introduced with Bitcoin \cite{Nakamoto:2008}. However, while Bitcoin aims to use the security of its immutable ledger to facilitate the exchange of coins among its users, Ethereum is proposed as a general-purpose global computer, in the sense that it enables developers to build and run \glspl{dapp} on its blockchain that maintains a single and globally accessible state. 

This state can be modified by running transactions related to two types of account: an \gls{eoa}, also known as a user account, stores and transacts Ethereum's native currency, \gls{eth}; and a \gls{sc} account, a contract account, acts as a repository for code, typically written in a Turing-complete high-level programming language (such as Solidity \cite{Solidity}) and stored in \gls{evm}~\cite{Antonopoulos:2018} bytecode form.

%acas: removi, pois não parece relevante para apresentar o problema de pesquisa a ser resolvido
%Only an \gls{eoa} can initiate a transaction on the Ethereum network. However, once initiated, this transaction can be directed either to another \gls{eoa} or to an \gls{sc} \cite{Wood:2014}. A special case occurs when a transaction is submitted to the network to create a new \gls{sc}. The destination of this type of transaction is set to null or contains the zero address (0×0) to indicate to the \gls{evm} that the bytecode contained within the transaction is the code for a new \gls{sc} intended to be deployed on Ethereum \cite{Antonopoulos:2018}.

%acas: idem acima
%When the destination of a transaction is an \gls{sc}, its bytecode must specify which function of the \gls{sc} is to be executed, as well as the arguments to be used in the call to the function. During its execution, the function may invoke functions from other \glspl{sc} by transmitting internal messages \cite{Liu:2020}.

Although Turing completeness enables the development of more complex and versatile applications, it also introduces the challenge of dealing with potentially unbounded loops. To prevent coding errors or malicious attacks from causing \glspl{sc} to run their code indefinitely, Ethereum has incorporated a \emph{gas system} that associates the cost of each computational operation on the blockchain (measured in gas units) with a specific amount of \textit{Wei} ($10^{-18}$ \gls{eth}) \cite{Bouraga:2020}.

The existence of a gas system poses an additional challenge for developers; 
%who want to create \glspl{sc} to be implemented on Ethereum. This is because, 
in addition to ensuring that their code works correctly%
% and is computationally viable and secure
, developers need to understand how this gas system works to make their \glspl{sc} as cost-efficient as possible. Associated with this need, it is important that developers are able to reliably estimate the \gls{gu} by their contracts to offer more transparency to users of applications that use such \glspl{sc} \cite{Wessling:2018}, identify and optimise code patterns that consume more gas than necessary \cite{Marchesi:2020}, and verify security risks associated with excessive gas consumption \cite{Grech:2018}.

%A \gls{dapp} is software whose back-end logic is executed by \glspl{sc} deployed on a blockchain, such as Ethereum \cite{Wessling:2018}. 
One of the main obstacles to the widespread adoption of \glspl{dapp} by users is the lack of transparency and predictability of the costs associated with \glspl{sc} that manage such applications \cite{AlShamsi:2022}. If developers can estimate the gas usage of their \glspl{sc}, they will be able to clearly present the expected cost for each interaction with these contracts. This level of transparency is essential, as users are more likely to interact with \glspl{dapp} when they are properly informed about their costs.

One of the main security issues associated with \gls{gu} transactions is the vulnerability arising from \gls{dos} attacks. Such attacks may exploit \glspl{sc} functions that do not adequately handle out-of-gas conditions. In these cases, the attacker can create multiple transactions that force a vulnerable function into an endless cycle of out-of-gas exceptions \cite{Grech:2018}. By estimating the gas used by their \glspl{sc}, developers can identify functions that consume significantly more gas units than expected, indicating suboptimal loops and security risks.

The Ethereum's gas system requires any user who wants to initiate a transaction to configure %the following 
several gas-related parameters. For our purpose here, we are particularly concerned with  \gls{gl} that 
%\gls{mpfg}, and \gls{mfg} \cite{EIP1559}. The \gls{gl} 
sets the maximum limit of gas units that can be consumed during the execution of a transaction. 
%The \gls{mpfg} and the \gls{mfg}, defined in \textit{Wei}, respectively determine the maximum tip amount that the transaction sender is willing to pay the validators (who are responsible for the inclusion of new blocks in the Ethereum network) and the total maximum amount the sender is willing to pay for the transaction execution. This total includes the tip and the \gls{bf}, which is automatically adjusted with every block to balance the demand for transactions and the supply of block space.
Before executing a transaction sent to an \gls{sc}, the \gls{evm} first verifies whether the transaction's \gls{gl} is, at least, equal to the \gls{igc}. However, this analysis ignores the cost associated with executing the code within the \gls{sc} (\gls{egc}), which can only be determined by the \gls{evm} at runtime \cite{Wood:2014}. Thus, if the sender sets the \gls{gl} to a value equal to or higher than the \gls{igc} but insufficient to cover the \gls{egc} of the \gls{sc}, the transaction will be prematurely terminated.

When a transaction is interrupted before being fully executed, the \gls{evm} raises an \gls{oge} and reverts the blockchain state to that immediately prior to the start of the transaction's execution. Furthermore, the \gls{gu} in its partial execution is not refunded, as the protocol does not allow for any refunds in such cases \cite{Antonopoulos:2018}. Thus, in addition to financial losses, \glspl{oge} can also expose \glspl{sc} to denial-of-service attacks and other types of vulnerabilities, as previously mentioned.  %\cite{Grech:2018}.

Correctly configuring the \gls{mgl} of a transaction is a particularly complex task because, on the one hand, underestimating the \gls{mgl} causes the transaction to be prematurely terminated, while on the other, its overestimation can exacerbate financial losses associated with bugs or attacks that can cause the \gls{sc} code to run indefinitely \cite{Marchesi:2020}. Furthermore, overestimating the \gls{mgl} can also lead the issuer to incorrectly configure the transaction's \gls{mpfg}, opting for a more conservative value than would be necessary if the \gls{mgl} had been accurately estimated. This occurs because the \gls{gl} is expected to be adjusted to achieve the best cost-benefit ratio between the transaction's \gls{mgl} and its validation time \cite{Zarir:2021}.

We were able to find only a few works that systematically address the challenges related to gas estimation in Ethereum transactions. These works propose gas estimators as a single solution for estimating both transaction \glspl{gu} and \glspl{mgl}, making no distinction between the two metrics. Liu et al. \cite{Liu:2020} categorise gas estimation methodologies into online and offline. According to this categorisation, offline estimators analyse the source code of \glspl{sc} to suggest the highest expected \gls{gu}/\gls{mgl} for each of its functions \cite{Albert:2020}. On the other hand, online estimators predict the \gls{gu}/\gls{mgl} of transactions based on data extracted from the Ethereum network or from a local blockchain operating under the same protocol \cite{Ma:2022}.

A known issue with offline gas estimators is their inability to effectively handle functions that feature loops with unknown termination criteria, as they rely solely on static code analysis \cite{Li:2020}. Moreover, the precision of such estimators tends to be compromised when they are applied to functions that include state variables in their scope. The reason is that the inclusion of state variables in a function's scope directly impacts its dependency on the blockchain's state, possibly affecting its \gls{gu} and \gls{mgl}.

From a different perspective, online gas estimators derive their predictions from the current state of the blockchain, making them inherently more accurate than their offline counterparts \cite{Liu:2020}. More specifically, these estimators can predict the \gls{gu}/\gls{mgl} of a given transaction by simulating its execution in an environment that emulates the updated state of the \gls{evm} \cite{Li:2020} or based on the \glspl{gu}/\glspl{mgl} of similar transactions that are already stored on the Ethereum blockchain \cite{Zarir:2021}.

Given the dynamic nature of Ethereum, the dependence on the current state of its blockchain poses a significant challenge for the implementation of online gas estimation techniques; the main difficulty lies in maintaining an updated representation of the state of the blockchain, since a new block is added to the Ethereum blockchain approximately every 12 seconds \cite{Ethereumdoc}.

A second challenge associated with online gas estimators arises when  the source code of the \glspl{sc} invoked by the analysed transactions is not considered. In these scenarios, the estimators do not have access to the peculiarities of the functions being called, and if they consider only the \gls{gu} by the transactions, they will be unable to identify situations where the internal logic of the \glspl{sc} demands that the \gls{mgl} allocated for the transaction's execution exceeds what is actually used.

%An Ethereum \gls{el} client is software designed to facilitate communication with the Ethereum platform \cite{Antonopoulos:2018}. This type of application is intended to listen for and process new transactions transmitted on the network, in addition to maintaining an updated version of the blockchain and the global state of the \gls{evm} \cite{Ethereumdoc}.

The formal specification of the Ethereum protocol requires \gls{el} clients to provide a built-in function, \textit{eth\_estimateGas()}, which is designed to estimate the \gls{mgl} of transactions \cite{Ethereumdoc}. Furthermore, the main \gls{el} clients~\cite{Gethdoc, Paritydoc, Netherminddoc, Erigondoc} implement another function, usually named \textit{debug\_traceCall()}, which aims to simulate the execution of transactions on the \gls{evm} without actually including them on the blockchain. This function, among other things, returns the \gls{gu} by such a transaction if it were entered into the blockchain under the same simulation conditions.
Both the \textit{debug\_traceCall()} and \textit{eth\_estimateGas()} functions can be categorized as online gas estimators, as they make their estimates based on the current state of the blockchain.

%acas: mover para outra seção, possivelmente a seção 3
%An important feature of the \textit{debug\_traceCall()} and \textit{eth\_estimateGas()} functions is that they have direct access to the updated copy of the blockchain preserved by the \gls{el} clients, thus eliminating the need for any other external representation of the state stored by the \gls{evm}. Furthermore, when it comes to estimating \gls{mgl}, the \textit{eth\_estimateGas()} function can effectively handle transactions that require \gls{mgl} values greater than the \gls{gu} by the functions called. This capability arises because this function operates by executing the transaction under analysis with various \gls{gl} values until it identifies the minimum value that guarantees the successful execution of the transaction \cite{Gethgit}.

We conduct an empirical study to evaluate the precision of the \textit{debug\_traceCall()} and \textit{eth\_estimateGas()} functions to answer the following research questions:

\textbf{\gls{rq1}}: \textbf{Under what circumstances is the \textit{eth\_estimateGas()} function expected to perform similarly to a perfect \glspl{mgl} estimator?}

% Our motivation for this question stems from the understanding that the \textit{eth\_estimateGas()} function works as a perfect estimator when predicting the \gls{mgl} of a transaction, provided that its arguments faithfully represent the attributes of the transaction and the current state of the blockchain at the time the transaction is included.

% To address this question, we designed an experiment aimed at identifying whether and to what extent the precision of \textit{eth\_estimateGas()} is affected by varying levels of delay between the blocks used to estimate the \glspl{mgl} and the blocks where the transactions were actually included.

% By bringing to light the precision of the \textit{eth\_estimateGas()} function, we aim to answer the extent to which users interacting with \glspl{sc} on Ethereum can trust the results of this function, to avoid underestimating or overestimating the \glspl{mgl} of their transactions and the problems that arise from these errors.

\textbf{\gls{rq2}}: \textbf{Under what circumstances is the \textit{debug\_traceCall()} function expected to perform similarly to a perfect \glspl{gu} estimator?}

% Similarly to \gls{rq1}, this question is motivated by the understanding that the \textit{debug\_traceCall()} function, when used as a \gls{gu} estimator, acts as a perfect estimator in predicting the \gls{gu} by a transaction, provided that its arguments accurately represent the transaction attributes and the current state of the blockchain at the time the transaction is included.

% To answer this question, we designed an experiment aimed at identifying whether and to what extent the precision of \textit{debug\_traceCall()} is affected by varying levels of delay between the blocks used to estimate the \glspl{gu} and the blocks where the transactions were actually included.

% By answering this question, our aim is to provide developers with reliable indicators of how much they can trust the results of the \textit{debug\_traceCall()} function, to provide more transparency to users of their \glspl{sc} and ensure the security of their code.

% \textbf{\gls{rq1}}: \textbf{How accurately is the \textit{debug\_traceCall()} function able to estimate the \glspl{gu} by transactions not yet included in the Ethereum blockchain?}

% The motivation for this research question comes from our finding that the \textit{debug\_traceCall()} function, when used as a \gls{gu} estimator, can provide more accurate results than currently available gas estimators, since being built into an \gls{el} client, it has direct access to an updated copy of the blockchain, as well as the current state of the \gls{evm}.

% By answering this question, our aim is to provide developers with reliable indicators of how much they can trust the results of the \textit{debug\_traceCall()} function, to provide more transparency to users of their \glspl{sc} and ensure the security of their code.

% \textbf{\gls{rq2}}: \textbf{How accurately is the \textit{eth\_estimateGas()} function able to estimate the \glspl{gl} of transactions not yet included in the Ethereum blockchain?}

% \textbf{\gls{rq2}}: \textbf{How accurately can we predict the \gls{mgl} of an Ethereum smart-contract-call transaction?}

% \textbf{\gls{rq2}}: \textbf{How accurate is the calculation of \gls{mgl} at blockchain state $\sigma$ as a prediction for this value at a later state $\sigma'$ for an Ethereum smart-contract-call transaction?}

%acas
% Given the \gls{mgl} (min) of an \gls{sc} transaction for a block K of an Ethereum blockchain, what is the precision of using min  as a prediction for a block at a distance \delta of k 

% \textbf{\gls{rq2}}: \textbf{For an Ethereum smart-contract-call transaction, how accurate is the \gls{mgl} at blockchain state $\sigma$ as an estimation for state $\sigma'$ ?}

% Our motivation for this question stems from the understanding that, similar to what happens with the \textit{debug\_traceCall()} function, direct access to the copy of the blockchain stored by \gls{el} clients provides the \textit{eth\_estimateGas()} function with a competitive advantage over other gas estimators. Furthermore, we expect that the \textit{eth\_estimateGas()} function to be able to estimate the \gls{gl} of transactions with greater precision than the gas estimators currently available, due to its ability to distinguish cases where the \gls{gl} of transactions is different from their \gls{gu}.

% By bringing to light the precision of the \textit{eth\_estimateGas()} function, we aim to answer the extent to which users interacting with \glspl{sc} on Ethereum can trust the results of this function, to avoid underestimating or overestimating the \glspl{gl} of their transactions and the problems that arise from these errors.

\textbf{\gls{rq3}}: \textbf{Are there significant differences between the \glspl{gu} and \glspl{mgl} of Ethereum \gls{sc} call transactions?}

Our motivation for \glspl{rq1} and \glspl{rq2} arises from the understanding that the \textit{eth\_estimateGas()} and \textit{debug\_traceCall()} functions act as perfect estimators when predicting, respectively, the \gls{mgl} and \gls{gu} of a transaction, provided that their arguments faithfully represent the transaction attributes and the current state of the blockchain at the time the transaction is included.

To address these research questions, we designed two experiments with the goal of identifying whether and to what extent the precision of \textit{eth\_estimateGas()} and \textit{debug\_traceCall()} is affected by varying levels of delay between the blocks used to make their estimates and the blocks where the transactions were actually included.

By highlighting the precision of the \textit{eth\_estimateGas()} and \textit{debug\_traceCall()} functions, we aim to clarify the extent to which users interacting with \glspl{sc} on Ethereum can rely on the results of these two functions. This understanding will enable users to make proper use of \textit{eth\_estimateGas()}, avoiding underestimation or overestimation of the \glspl{mgl} of their transactions and preventing problems arising from these errors. Additionally, by utilizing \textit{debug\_traceCall()}, they will be able to ensure greater transparency for the users of their \glspl{sc} and enhance the security of their code.

\gls{rq3} derives from the observation that, as far as we are concerned, none of the works proposing new gas estimators makes a clear distinction between the \glspl{gu} and \glspl{mgl} of the transactions. Based on this, we understand that significant differences between transaction \glspl{gu} and \glspl{mgl} can negatively affect the precision of currently available gas estimators.

Our objective in answering this question is to provide insight so that the community of researchers and developers working with gas estimation on Ethereum understands how much differences between transaction \glspl{gu} and \glspl{mgl} could impact their estimators.

%We have structured the remaining sections of the article as follows:
%\begin{itemize}
Section~\ref{section:background} briefly introduces the main concepts of blockchains, \glspl{sc}, and the Ethereum gas system. Section~\ref{section:minimum-gas-limit-vs-gas-used} defines and explains the differences between the \gls{mgl} and the \gls{gu} in an Ethereum transaction. To answer the research questions posed in this paper, in Section~\ref{section:evaluation} an experimental design and the related results are presented.  
Section \ref{section:related-work} discusses works related to the topic of our research. The final section
%\ref{section:conclusions}
summarises our conclusions and outlines open areas for future research.

%\end{itemize}
